On-Chip Characterization of High-Loss Liquids between 750 GHz and 1100 GHz

Terahertz spectroscopy is a promising tool for analyzing the picosecond dynamics of biomolecules, which is influenced by surrounding water molecules. However, water causes extreme losses to terahertz signals, preventing sensitive measurements at this frequency range. Here, we present sensitive on-chip terahertz spectroscopy of highly lossy aqueous solutions using a vector network analyzer, contact probes, and a coplanar waveguide with a 0.1 mm wide microfluidic channel. The complex permittivities of various deionized water/isopropyl alcohol concentration are extracted from a known reference measurement across the frequency range 750-1100 GHz and agrees well with literature data. The results prove the presented method as a high-sensitive approach for on-chip terahertz spectroscopy of high-loss liquids, capable of resolving the permittivity of water.

==> Settings.tex <==
% BASIC SETTINGS
\usepackage{caption}
\usepackage{commath}
\usepackage{graphicx, epstopdf}                                                           % Figures
\usepackage{longtable}
\usepackage{mwe}
\setlength{\parskip}{0em}
\usepackage{subcaption}

\usepackage{moreverb}                                                           % List settings
\usepackage{textcomp}                                                           % Fonts, symbols etc.
\usepackage{lmodern}                                                            % Latin modern font
\usepackage{helvet}                                                             % Enables font switching
\usepackage[T1]{fontenc}                                                        % Output settings
%\usepackage[swedish]{babel}                                                    % Language settings
\usepackage[utf8]{inputenc}                                                     % Input settings
\usepackage{amsmath}                                                            % Mathematical expressions (American mathematical society)
\usepackage{amssymb}                                                            % Mathematical symbols (American mathematical society)
\usepackage{subfig}                                                                     % Enables subfigures
\usepackage{listings}                                                           % Enables source code listings
\usepackage{chemfig}                                                    % Chemical structures
\usepackage{siunitx}
\usepackage[a4paper, total={15cm, 23.7cm}]{geometry}
%\usepackage[top=3cm, bottom=3cm,inner=3cm, outer=3cm]{geometry}                 % Page margin lengths                  
\usepackage{eso-pic}                                                            % Create cover page background
\newcommand{\backgroundpic}[3]{
        \put(#1,#2){
        \parbox[b][\paperheight]{\paperwidth}{
        \centering
        \includegraphics[width=0.8\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
       
        
\usepackage{csquotes}
\usepackage{filecontents} 

%

% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)
%\usepackage{color}
\usepackage{comment}
\usepackage{lipsum}
\usepackage{float}
\usepackage{hyperref}
\usepackage{pgfgantt}
\usepackage{etoolbox}
\usepackage{placeins}
\usepackage{xpatch}
\usepackage{siunitx}
\usepackage[super]{nth}
\usepackage{titlesec}
\usepackage{pdfpages}
\usepackage[numbers]{natbib}
\usepackage{units}

%% MATLAB-code fix

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Matlab,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbersf
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}


\epstopdfsetup{outdir=./}
\graphicspath{{./fig/}}

==> include/Papers_to_cite.tex <==
\section{Papers to cite}

\begin{itemize} 
    \item "Terahertz Microfluidic Metamaterial Biosensor for Tiny Volume Liquid Samples" \cite{Zhang2019a}
\end{itemize}

